IoT-Scan: Network Reconnaissance for the Internet of Things

Network reconnaissance is a core networking and security procedure aimed at discovering devices and their properties. For IP-based networks, several network reconnaissance tools are available, such as Nmap. For the Internet of Things (IoT), there is currently no similar tool capable of discovering devices across multiple protocols. In this paper, we present IoT-Scan, a universal IoT network reconnaissance tool. IoT-Scan is based on software defined radio (SDR) technology, which allows for a flexible software-based implementation of radio protocols. We present a series of passive, active, multi-channel, and multi-protocol scanning algorithms to speed up the discovery of devices with IoT-Scan. We benchmark the passive scanning algorithms against a theoretical traffic model based on the non-uniform coupon collector problem. We implement the scanning algorithms and compare their performance for four popular IoT protocols: Zigbee, Bluetooth LE, Z-Wave, and LoRa. Through extensive experiments with dozens of IoT devices, we demonstrate that our implementation experiences minimal packet losses and achieves performance near the theoretical benchmark. Using multi-protocol scanning, we further demonstrate a reduction of 70\% in the discovery times of Bluetooth and Zigbee devices in the 2.4\,GHz band and of LoRa and Z-Wave devices in the 900\,MHz band, compared to sequential passive scanning. We make our implementation and data available to the research community to allow independent replication of our results and facilitate further development of the tool.

==> 07_limitations.tex <==
\section{Limitations and Future Work}
In this study Zigbee active scan discovers a dozen devices in about 50\% less time than passive scan does. The benefit of active scan will grow with increasing size of the network. On the other hand, the probability of colliding beacons increases due to multiple responses (single coordinator and all routers will reply with beacons on a single channel).

To reduce the collisions due to multiple responses one could actively scan with directed or non-broadcasting probe requests (as they are called in Wi-Fi).
One way to implement directed probe requests is using the fact that devices from different chipset vendors have different reception rates to non-standard preambles and SFDs (starting frame delimiter)
In \cite{jaakkola2007usage} Wi-Fi active scan reduces collisions due to multiple responses by sending directed probe requests sequentially, i.e. closely one after the other.


%In Zigbee, we use beacon requests for active scanning as they are broadcast to all devices without requiring prior knowledge of destination addresses. Assuming prior knowledge of all device addresses (such as after one initial complete detection scan), active scanning could potentially be further sped up by using association requests (which use unicast addressing and therefore require individual requests per target device) to perform active scan.

==> sections/acknowledgement.tex <==
\section*{Acknowledgment}
The authors would like to thank ... for his/her/their help and support during the process of writing this paper. 

==> sections/discussion.tex <==
\section{Discussion}
\label{section:disc}
Here you can discuss your results, limitations and new questions that have arose while doing the work. Depending on the size of this report, you can present discussion and conclusion in one common section or in two separate ones. 

==> sections/keywords.tex <==
\begin{center}
\begin{IEEEkeywords}
Alphabetical, Be, In, Order, Should
\end{IEEEkeywords}
\end{center}

==> sections/method.tex <==
\section{Method}
\label{section:method}
In this section, the method used to find an answer to the research questions should be presented. 

If this report presents results from a literature search, this means providing sufficient information for allowing someone else to repeat the literature search and compare the results. I.e., a search using the phrases a, b, and c, was made in database x, y and z on the date Month Date, Year (e.g., July 31st, 2021). The search resulted in x hits. Then, information on how you chose which works to include in this report should be provided. The references should be used for answering your research questions.

If the work reports on an experiment, this part should provide information about the experimental setup, how the experiment was conducted, how data was collected and analyzed etc. Motivate methodological choices through references. Also an experiment should be presented with sufficient detail such that it can be repeated by someone else.

==> sections/results.tex <==
\section{Results}
\label{section:results}
This section should present answers to all research questions.

It is normal to have only one results section, but you can create more sections if finding it more appropriate. You can also divide results into subsections. Perhaps you want to refer to some other section, for example (see Section \ref{section:method}). You can also place figures, you should always reference these in the text, see Figure \ref{fig:MDHlogga} for an example of a figure including subfigures. Remember that all figures should have a figure label explaining their content.


\begin{figure}[H]
    \centering
    \subfigure[MDH logo]{
    \label{fig:MDH1}
    \includegraphics[width=.2\columnwidth]{MDHlogga}}
    \qquad
    \subfigure[MDH logo]{
    \label{fig:MDH2}
    \includegraphics[width=.2\columnwidth]{MDHlogga}}
    \qquad
    \subfigure[MDH logo]{
    \label{fig:MDH3}
    \includegraphics[width=.2\columnwidth]{MDHlogga}}
    \caption[Short text]{This is a example of multiple figures.}
    \label{fig:MDHlogga}
\end{figure}
